A general method for estimating the prevalence of Influenza-Like-Symptoms with Wikipedia data

Influenza is an acute respiratory seasonal disease that affects millions of people worldwide and causes thousands of deaths in Europe alone. Being able to estimate in a fast and reliable way the impact of an illness on a given country is essential to plan and organize effective countermeasures, which is now possible by leveraging unconventional data sources like web searches and visits. In this study, we show the feasibility of exploiting information about Wikipedia's page views of a selected group of articles and machine learning models to obtain accurate estimates of influenza-like illnesses incidence in four European countries: Italy, Germany, Belgium, and the Netherlands. We propose a novel language-agnostic method, based on two algorithms, Personalized PageRank and CycleRank, to automatically select the most relevant Wikipedia pages to be monitored without the need for expert supervision. We then show how our model is able to reach state-of-the-art results by comparing it with previous solutions.

==> imports/draft.tex <==
%!TEX root = ../wikiflu-acm.tex

% Required packages
\usepackage[dirty=DirtyRepo]{gitinfo2}
\usepackage{etoolbox}
\usepackage{keyval}
\usepackage{xstring}
\usepackage{background}
\usepackage[yyyymmdd,hhmmss]{datetime}

\global\newtoggle{isDraft}

\makeatletter
% How to create a command with key values?
% https://tex.stackexchange.com/a/34314/25748
% ========= KEY DEFINITIONS =========
\define@key{draft}{position}{\def\pb@position{#1}}
\define@key{draft}{vshift}{\def\pb@vshift{#1}}
\define@key{draft}{hshift}{\def\pb@hshift{#1}}
\define@key{draft}{scale}{\def\pb@scale{#1}}
% ========= KEY DEFAULTS =========
\setkeys{draft}{position=current page.west,vshift=-0.5\leftmargin,hshift=0.3\textheight,scale=2}%
\newcommand{\draft}[2][]{%
  \global\toggletrue{isDraft}%

  % Set new keys
  \setkeys{draft}{#1}

  % use dashes as separators for dates (default in git, so it is needed for
  % consistency)
  \renewcommand{\dateseparator}{-}

  % define watermark color
  \definecolor{draftwatermarkcolor}{HTML}{E00116}

  % define \gitBranchSymbol: start from \hookrightarrow, rotate it 45 degrees
  % and scale it by 1.2 times
  \newcommand{\rotatedhookrightarrow}{\mathpalette{\rotatebox[origin=c]{45}{$\hookrightarrow$}}\relax}%
  \newcommand{\gitBranchSymbol}{$\scalebox{1.2}{\ensuremath{\rotatedhookrightarrow}}$}%

  % if the repo is dirty we put the symbol otherwise we leave it empty
  \newcommand{\gitIfIsDirtyRepoSymbol}{\IfSubStr{\gitDirty}{DirtyRepo}{\gitBranchSymbol}{}}

  % define \gitCommitterDateTime (date and time of last commit) from
  % \gitCommitterIsoDate: 19 is a magic number: 'yyyy-mm-dd hh:MM:ss' has
  % length 19.
  \StrSplit{\gitCommitterIsoDate}{19}{\gitCommitterDateTime}{}

  % if the option "long" is passed then the commit is dispalied with date and
  % time otherwise only date.
  \newcommand{\gitCommitterDateDisplay}{\IfSubStr{#2}{long}{\gitCommitterDateTime}{\gitCommitterDate}}

  \newcommand{\gitAuthor}{\StrCut{\gitAuthorName}{ }{\csName}{\csSurname}\csName}

  \usepackage{amssymb}
  \newcommand{\gitRelInfo}{\IfEq{\gitRoff}{}{$\diamond$-\gitRel}{\gitRel-\gitRoff}}

  % watermark text
  \newcommand{\drafttext}{DRAFT (v. \gitIfIsDirtyRepoSymbol\gitAbbrevHash, \gitAuthor, \gitRelInfo, \gitCommitterDateDisplay) ~\today ~\currenttime}

  \backgroundsetup{contents=\drafttext,%
           color=draftwatermarkcolor,
           opacity=1,%
           angle=90,%
           position=\pb@position,%
           vshift=\pb@vshift,%
           hshift=\pb@hshift,%
           scale=\pb@scale%
  }%
  \pagenumbering{arabic}%
}
\makeatother


==> imports/hyphenation.tex <==
% define special cases for hyphenation
\hyphenation{da-ta-ba-se}
\hyphenation{me-thodo-lo-gies}
\hyphenation{se-man-tics}
\hyphenation{dif-fer-ent}
\hyphenation{de-no-tes}
\hyphenation{re-spec-tive-ly}
\hyphenation{at-tribute}


==> imports/notes.tex <==
% the toggle isDraft is defined in draft.tex
\iftoggle{isDraft}{%
  \usepackage[show]{chato-notes}
}{%
  \usepackage[hide]{chato-notes}
}

